The Convolution Series Solution of Divergent Navier-Stokes Equations

This paper gives out the solution of divergent Navier-Stokes equations, and shows that in this case, under a physicalacceptable condition, the solution would be smooth .

==> 0302898.tex <==
%auto-ignore
